FashionTex: Controllable Virtual Try-on with Text and Texture

Virtual try-on attracts increasing research attention as a promising way for enhancing the user experience for online cloth shopping. Though existing methods can generate impressive results, users need to provide a well-designed reference image containing the target fashion clothes that often do not exist. To support user-friendly fashion customization in full-body portraits, we propose a multi-modal interactive setting by combining the advantages of both text and texture for multi-level fashion manipulation. With the carefully designed fashion editing module and loss functions, FashionTex framework can semantically control cloth types and local texture patterns without annotated pairwise training data. We further introduce an ID recovery module to maintain the identity of input portrait. Extensive experiments have demonstrated the effectiveness of our proposed pipeline.

==> Figs/modulation.tex <==
\begin{figure}
    \vspace{-1mm}
  \centering
  %\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   \includegraphics[width=\linewidth]{Imgs/modulation.png}

    \vspace{-1mm}
   \caption{The modulation module. }
   \label{fig:modulation}
   \vspace{-1mm}
\end{figure}

==> Figs/teaser.tex <==
\begin{center}
\centering
 \vspace{-1mm}
  \captionsetup{type=figure}
  %\fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
  \includegraphics[width=\linewidth]{Imgs/new_teaser.pdf}
\captionof{figure}{FashionTex performs the full-body virtual try-on with multi-modal
controls over garment type and texture pattern, allowing anyone to design personalized clothes with simple interactions. We show two design cases here. For each of the cases, the input portrait is presented on the left, with three outputs under different conditions. Each condition contains one text prompt and two texture patches for upper and lower cloth parts.} 
    \vspace{-1mm}
   \label{fig:teaser}
   \vspace{-1mm}
    
\end{center}

% Put the teaser under authors
%\twocolumn[{%
%\renewcommand\twocolumn[1][]{#1}%
%\maketitle
%\begin{center}
%    \centering
%    \captionsetup{type=figure}
%    \includegraphics[width=0.9\textwidth]{imgs/fig_intro_1.png}
%    \captionof{figure}{Test caption} \label{fig:information_density}
%\end{center}%
%}]

==> Tables/quant_0.tex <==
\begin{table*}[htbp]
  % \renewcommand\tabcolsep{5pt} 
  \centering
   \footnotesize
  \caption{}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{tabular}{|l|l|ll|l|l|ll|}
                   Task   & Method     & FID & LPIPS &                  Task        & Method            & FID & Accuracy \\ \hline
Type & TextureGAN &     &       & 
Texture & TextureGAN        &     &          \\
                      & Styleclip  &     &       &                          & Texture Reformer  &     &          \\
                      & Tedigan    &     &       &                          & Dressing in order &     &          \\
                      & Ours       &     &       &                          & Ours              &     &         
\end{tabular}
\end{table*}

==> Tables/user_study.tex <==




\begin{table}[t]
\small
\centering
\tabcolsep 2pt
 \caption{Results of user study. Above: type editing. Below: texture transfer. \todo{Same as the above table}}
  \begin{tabular}{l|c|ccc}
  \hline
  &  Method & Realism $\uparrow$ & Preservation $\uparrow$ & Consistence $\uparrow$ \\
  \hline
   \multirow{3}*{Type}
 
		&  Styleclip\cite{patashnik2021styleclip} & 32 & 32\\
		&  Tedigan\cite{xia2021tedigan} & 64 & 32 \\
		&  Ours & 32 & C  \\
\hline
\hline
   \multirow{4}*{Texture}
 
   	&  TextureGAN\cite{xian2018texturegan} & 32 & 0.4232 \\
		&  Texture Reformer\cite{wang2022texture} & 32 & 0.3687\\
		&  DiOr\cite{cui2021dressing} & 64 & 0.3784 \\
		&  Ours & 32 & 0.3257  \\
		\hline
	\end{tabular}
\label{tab:userstudy}
\end{table}

